How to define a context-free backbone for DGs: Implementing a DG in the LFG formalism

This paper presents a multidimensional Dependency Grammar (DG), which decouples the dependency tree from word order, such that surface ordering is not determined by traversing the dependency tree. We develop the notion of a \emph{word order domain structure}, which is linked but structurally dissimilar to the syntactic dependency tree. We then discuss the implementation of such a DG using constructs from a unification-based phrase-structure approach, namely Lexical-Functional Grammar (LFG). Particular attention is given to the analysis of discontinuities in DG in terms of LFG's functional uncertainty.

==> nobi-hyphen.tex <==
\hyphenation{
Hash-funk-tion
Hash-funk-tio-nen
Dis-kurs-wissen
Teil-auf-gabe
beruf-liche
Unifikations-formalis-mus
buch-staben-orien-tierten
an-dere
Sys-tems
Nomina
Allo-morphie
Wort-analysen
aus-gehend
be-deutungs-tragende
Lexikon-organi-sation
Analyse-protokoll
Wort-seman-tik
%re-pr"asentiert
Kombi-nations-regeln
Kate-gorien
De-fini-tion
spe-zielle
% Pr"afixe
Im-ple-men-tation
buch-staben-orien-tiert
Adjektiv-endun-gen
Allo-morph-re-geln
TRUE
Pro-gramm
Kla-ssi-fi-ka-tion
Sprach-ana-lyse-sys-tem
morphem-orientiert
Ana-lyse-pro-gramm
ka-te-go-ri-siert
regexp
Allo-morphe
Lama
Haupt-speicher
dies
Parti-zipI
Para-digma
be-nutzt
}

